Direct and indirect evidence of compression of word lengths. Zipf's law of abbreviation revisited

Zipf's law of abbreviation, the tendency of more frequent words to be shorter, is one of the most solid candidates for a linguistic universal, in the sense that it has the potential for being exceptionless or with a number of exceptions that is vanishingly small compared to the number of languages on Earth. Since Zipf's pioneering research, this law has been viewed as a manifestation of a universal principle of communication, i.e. the minimization of word lengths, to reduce the effort of communication. Here we revisit the concordance of written language with the law of abbreviation. Crucially, we provide wider evidence that the law holds also in speech (when word length is measured in time), in particular in 46 languages from 14 linguistic families. Agreement with the law of abbreviation provides indirect evidence of compression of languages via the theoretical argument that the law of abbreviation is a prediction of optimal coding. Motivated by the need of direct evidence of compression, we derive a simple formula for a random baseline indicating that word lengths are systematically below chance, across linguistic families and writing systems, and independently of the unit of measurement (length in characters or duration in time). Our work paves the way to measure and compare the degree of optimality of word lengths in languages.

==> references.tex <==
% https://tex.stackexchange.com/questions/34155/autoref-does-not-capitalize-initial-character-in-sentence-when-referencing-labe

\usepackage{catoptions}

\makeatletter
\def\figureautorefname{figure}
\def\tableautorefname{table}
\def\Autoref#1{%
  \begingroup
  \edef\reserved@a{\cpttrimspaces{#1}}%
  \ifcsndefTF{r@#1}{%
    \xaftercsname{\expandafter\testreftype\@fourthoffive}
      {r@\reserved@a}.\\{#1}%
  }{%
    \ref{#1}%
  }%
  \endgroup
}
\def\testreftype#1.#2\\#3{%
  \ifcsndefTF{#1autorefname}{%
    \def\reserved@a##1##2\@nil{%
      \uppercase{\def\ref@name{##1}}%
      \csn@edef{#1autorefname}{\ref@name##2}%
      \autoref{#3}%
    }%
    \reserved@a#1\@nil
  }{%
    \autoref{#3}%
  }%
}
\makeatother


==> tables/cvVSpud_k.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Thu Jun 30 16:39:57 2022
1.00 & 1.00 & 1.00 & 1.00 &   2 & 5569590 \\ 
  -0.33 & 1.00 & 1.00 & 0.33 &   3 & 5014779 \\ 
  -0.33 & 0.75 & 0.67 & 0.33 &   4 & 4339527 \\ 
  -0.20 & 0.82 & 0.80 & 0.08 &   5 & 2673259 \\ 
  -0.07 & 1.00 & 0.73 & 0.06 &   6 & 2484983 \\ 
  -0.24 & 0.56 & 0.62 & 0.07 &   7 & 2278604 \\ 
  0.07 & 0.90 & 0.43 & 0.18 &   8 & 1052514 \\ 
  0.11 & 0.76 & 0.50 & 0.08 &   9 & 830059 \\ 
  0.07 & 0.86 & 0.60 & 0.02 &  10 & 826468 \\ 
  -0.02 & 1.00 & 0.56 & 0.02 &  11 & 726539 \\ 
  0.12 & 0.64 & 0.45 & 0.04 &  12 & 647545 \\ 
  0.26 & 0.25 & 0.31 & 0.16 &  13 & 580778 \\ 


==> tables/cv_opt_scores_characters_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jul 11 12:37:22 2022
 Maltese & Afro-Asiatic & Latin & 3.71 & 5.07 & 7.34 & -0.19 & -0.81 & 0.73 & 0.62 & 0.24 \\ 
  Vietnamese & Austroasiatic & Latin & 2.70 & 3.22 & 3.40 & -0.16 & -0.72 & 0.84 & 0.26 & 0.22 \\ 
  Indonesian & Austronesian & Latin & 3.69 & 5.38 & 7.24 & -0.20 & -0.91 & 0.69 & 0.52 & 0.22 \\ 
  Esperanto & Conlang & Latin & 3.23 & 4.83 & 7.72 & -0.17 & -0.92 & 0.67 & 0.64 & 0.19 \\ 
  Interlingua & Conlang & Latin & 3.39 & 4.50 & 7.42 & -0.23 & -0.79 & 0.75 & 0.73 & 0.29 \\ 
  Tamil & Dravidian & Tamil & 4.60 & 5.72 & 7.02 & -0.26 & -0.87 & 0.80 & 0.54 & 0.30 \\ 
  Persian & Indo-European & Arabic & 2.64 & 3.80 & 5.49 & -0.20 & -0.92 & 0.69 & 0.59 & 0.22 \\ 
  Assamese & Indo-European & Assamese & 4.24 & 4.71 & 5.50 & -0.30 & -0.66 & 0.90 & 0.63 & 0.46 \\ 
  Russian & Indo-European & Cyrillic & 4.05 & 6.31 & 9.00 & -0.13 & -0.94 & 0.64 & 0.54 & 0.14 \\ 
  Ukrainian & Indo-European & Cyrillic & 4.53 & 5.52 & 7.67 & -0.16 & -0.86 & 0.82 & 0.68 & 0.19 \\ 
  Panjabi & Indo-European & Devanagari & 3.60 & 3.73 & 3.94 & -0.34 & -0.48 & 0.97 & 0.62 & 0.71 \\ 
  Modern Greek & Indo-European & Greek & 3.62 & 4.85 & 7.64 & -0.24 & -0.85 & 0.74 & 0.69 & 0.29 \\ 
  Breton & Indo-European & Latin & 2.88 & 3.98 & 6.32 & -0.24 & -0.90 & 0.72 & 0.68 & 0.26 \\ 
  Catalan & Indo-European & Latin & 2.98 & 4.90 & 8.58 & -0.15 & -0.92 & 0.61 & 0.66 & 0.17 \\ 
  Czech & Indo-European & Latin & 3.80 & 4.85 & 7.16 & -0.22 & -0.92 & 0.78 & 0.69 & 0.24 \\ 
  Dutch & Indo-European & Latin & 3.24 & 4.76 & 8.27 & -0.27 & -0.95 & 0.68 & 0.70 & 0.29 \\ 
  English & Indo-European & Latin & 2.36 & 4.61 & 7.79 & -0.07 & -0.83 & 0.51 & 0.59 & 0.09 \\ 
  French & Indo-European & Latin & 2.55 & 5.04 & 8.11 & -0.04 & -0.84 & 0.51 & 0.55 & 0.04 \\ 
  German & Indo-European & Latin & 2.91 & 5.73 & 10.28 & -0.11 & -0.87 & 0.51 & 0.62 & 0.13 \\ 
  Irish & Indo-European & Latin & 3.02 & 4.22 & 6.59 & -0.21 & -0.93 & 0.72 & 0.66 & 0.23 \\ 
  Italian & Indo-European & Latin & 3.13 & 5.29 & 8.15 & -0.05 & -0.90 & 0.59 & 0.57 & 0.06 \\ 
  Latvian & Indo-European & Latin & 4.00 & 4.84 & 7.09 & -0.25 & -0.73 & 0.83 & 0.73 & 0.35 \\ 
  Polish & Indo-European & Latin & 3.82 & 5.27 & 7.87 & -0.17 & -0.94 & 0.72 & 0.64 & 0.18 \\ 
  Portuguese & Indo-European & Latin & 3.15 & 4.61 & 7.49 & -0.18 & -0.91 & 0.68 & 0.66 & 0.20 \\ 
  Romanian & Indo-European & Latin & 3.61 & 5.03 & 7.67 & -0.21 & -0.78 & 0.72 & 0.65 & 0.27 \\ 
  Romansh & Indo-European & Latin & 3.81 & 4.94 & 7.53 & -0.23 & -0.79 & 0.77 & 0.70 & 0.29 \\ 
  Slovenian & Indo-European & Latin & 3.64 & 4.56 & 6.43 & -0.21 & -0.87 & 0.80 & 0.67 & 0.24 \\ 
  Spanish & Indo-European & Latin & 2.69 & 5.01 & 7.91 & -0.03 & -0.91 & 0.54 & 0.56 & 0.03 \\ 
  Swedish & Indo-European & Latin & 3.09 & 4.05 & 6.89 & -0.28 & -0.90 & 0.76 & 0.75 & 0.31 \\ 
  Welsh & Indo-European & Latin & 2.76 & 4.17 & 7.00 & -0.20 & -0.91 & 0.66 & 0.67 & 0.22 \\ 
  Western Frisian & Indo-European & Latin & 3.43 & 4.38 & 7.99 & -0.28 & -0.80 & 0.78 & 0.79 & 0.36 \\ 
  Oriya & Indo-European & Odia & 3.78 & 4.31 & 5.44 & -0.32 & -0.70 & 0.88 & 0.68 & 0.46 \\ 
  Dhivehi & Indo-European & Thaana & 2.16 & 3.50 & 7.74 & -0.23 & -0.82 & 0.62 & 0.76 & 0.28 \\ 
  Georgian & Kartvelian & Georgian & 6.01 & 7.27 & 8.24 & -0.11 & -0.67 & 0.83 & 0.43 & 0.17 \\ 
  Basque & Language isolate & Latin & 4.44 & 6.41 & 8.89 & -0.16 & -0.91 & 0.69 & 0.56 & 0.18 \\ 
  Mongolian & Mongolic & Mongolian & 4.19 & 5.48 & 7.32 & -0.22 & -0.86 & 0.76 & 0.59 & 0.26 \\ 
  Kinyarwanda & Niger-Congo & Latin & 3.69 & 6.13 & 9.19 & -0.19 & -0.90 & 0.60 & 0.56 & 0.21 \\ 
  Hakha Chin & Sino-Tibetan & Latin & 2.56 & 3.30 & 5.29 & -0.29 & -0.81 & 0.78 & 0.73 & 0.35 \\ 
  Chuvash & Turkic & Cyrillic & 5.00 & 6.26 & 7.53 & -0.20 & -0.83 & 0.80 & 0.50 & 0.25 \\ 
  Kirghiz & Turkic & Cyrillic & 4.51 & 6.04 & 7.81 & -0.19 & -0.89 & 0.75 & 0.54 & 0.22 \\ 
  Tatar & Turkic & Cyrillic & 4.05 & 5.43 & 7.47 & -0.24 & -0.88 & 0.75 & 0.60 & 0.27 \\ 
  Yakut & Turkic & Cyrillic & 5.01 & 6.32 & 7.98 & -0.26 & -0.74 & 0.79 & 0.56 & 0.35 \\ 
  Turkish & Turkic & Latin & 4.58 & 6.00 & 8.08 & -0.22 & -0.89 & 0.76 & 0.59 & 0.24 \\ 
  Estonian & Uralic & Latin & 4.68 & 6.20 & 8.84 & -0.23 & -0.83 & 0.75 & 0.63 & 0.28 \\ 
   \hline


==> tables/cv_opt_scores_medianDuration_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jul 11 12:37:22 2022
 Maltese & Afro-Asiatic & Latin & 0.26 & 0.35 & 0.54 & -0.21 & -0.81 & 0.74 & 0.68 & 0.26 \\ 
  Vietnamese & Austroasiatic & Latin & 0.22 & 0.30 & 0.34 & -0.06 & -0.78 & 0.72 & 0.30 & 0.08 \\ 
  Indonesian & Austronesian & Latin & 0.27 & 0.38 & 0.52 & -0.22 & -0.91 & 0.72 & 0.58 & 0.24 \\ 
  Esperanto & Conlang & Latin & 0.35 & 0.49 & 0.81 & -0.18 & -0.91 & 0.71 & 0.69 & 0.20 \\ 
  Interlingua & Conlang & Latin & 0.33 & 0.40 & 0.69 & -0.23 & -0.78 & 0.80 & 0.78 & 0.30 \\ 
  Tamil & Dravidian & Tamil & 0.46 & 0.55 & 0.67 & -0.30 & -0.86 & 0.85 & 0.59 & 0.35 \\ 
  Persian & Indo-European & Arabic & 0.26 & 0.36 & 0.54 & -0.25 & -0.99 & 0.72 & 0.65 & 0.25 \\ 
  Assamese & Indo-European & Assamese & 0.37 & 0.44 & 0.51 & -0.21 & -0.67 & 0.84 & 0.50 & 0.31 \\ 
  Russian & Indo-European & Cyrillic & 0.30 & 0.42 & 0.60 & -0.15 & -0.94 & 0.71 & 0.60 & 0.15 \\ 
  Ukrainian & Indo-European & Cyrillic & 0.37 & 0.43 & 0.59 & -0.17 & -0.86 & 0.85 & 0.72 & 0.20 \\ 
  Panjabi & Indo-European & Devanagari & 0.66 & 0.71 & 0.74 & -0.20 & -0.44 & 0.93 & 0.42 & 0.46 \\ 
  Modern Greek & Indo-European & Greek & 0.29 & 0.38 & 0.63 & -0.21 & -0.84 & 0.76 & 0.72 & 0.26 \\ 
  Breton & Indo-European & Latin & 0.22 & 0.31 & 0.52 & -0.25 & -0.88 & 0.71 & 0.70 & 0.28 \\ 
  Catalan & Indo-European & Latin & 0.24 & 0.36 & 0.68 & -0.21 & -0.94 & 0.67 & 0.73 & 0.23 \\ 
  Czech & Indo-European & Latin & 0.31 & 0.38 & 0.57 & -0.21 & -0.92 & 0.81 & 0.73 & 0.23 \\ 
  Dutch & Indo-European & Latin & 0.22 & 0.30 & 0.56 & -0.27 & -0.95 & 0.75 & 0.78 & 0.29 \\ 
  English & Indo-European & Latin & 0.19 & 0.33 & 0.67 & -0.17 & -0.83 & 0.58 & 0.71 & 0.21 \\ 
  French & Indo-European & Latin & 0.19 & 0.32 & 0.63 & -0.21 & -0.85 & 0.58 & 0.69 & 0.25 \\ 
  German & Indo-European & Latin & 0.23 & 0.37 & 0.76 & -0.21 & -0.87 & 0.63 & 0.74 & 0.25 \\ 
  Irish & Indo-European & Latin & 0.22 & 0.30 & 0.47 & -0.23 & -0.92 & 0.76 & 0.70 & 0.25 \\ 
  Italian & Indo-European & Latin & 0.26 & 0.38 & 0.65 & -0.19 & -0.90 & 0.69 & 0.70 & 0.21 \\ 
  Latvian & Indo-European & Latin & 0.33 & 0.39 & 0.59 & -0.23 & -0.73 & 0.84 & 0.77 & 0.31 \\ 
  Polish & Indo-European & Latin & 0.30 & 0.38 & 0.57 & -0.17 & -0.95 & 0.79 & 0.71 & 0.18 \\ 
  Portuguese & Indo-European & Latin & 0.27 & 0.36 & 0.62 & -0.21 & -0.92 & 0.76 & 0.75 & 0.23 \\ 
  Romanian & Indo-European & Latin & 0.27 & 0.36 & 0.57 & -0.23 & -0.77 & 0.74 & 0.69 & 0.30 \\ 
  Romansh & Indo-European & Latin & 0.33 & 0.41 & 0.66 & -0.26 & -0.78 & 0.81 & 0.77 & 0.33 \\ 
  Slovenian & Indo-European & Latin & 0.36 & 0.44 & 0.63 & -0.25 & -0.85 & 0.83 & 0.71 & 0.29 \\ 
  Spanish & Indo-European & Latin & 0.21 & 0.36 & 0.62 & -0.13 & -0.91 & 0.58 & 0.64 & 0.15 \\ 
  Swedish & Indo-European & Latin & 0.22 & 0.27 & 0.52 & -0.29 & -0.90 & 0.81 & 0.83 & 0.33 \\ 
  Welsh & Indo-European & Latin & 0.22 & 0.32 & 0.58 & -0.20 & -0.93 & 0.69 & 0.72 & 0.21 \\ 
  Western Frisian & Indo-European & Latin & 0.26 & 0.32 & 0.61 & -0.31 & -0.80 & 0.80 & 0.82 & 0.39 \\ 
  Oriya & Indo-European & Odia & 0.36 & 0.41 & 0.50 & -0.32 & -0.70 & 0.89 & 0.69 & 0.46 \\ 
  Dhivehi & Indo-European & Thaana & 0.18 & 0.35 & 0.79 & -0.17 & -0.80 & 0.50 & 0.71 & 0.21 \\ 
  Georgian & Kartvelian & Georgian & 0.45 & 0.53 & 0.61 & -0.14 & -0.65 & 0.85 & 0.50 & 0.22 \\ 
  Basque & Language isolate & Latin & 0.33 & 0.44 & 0.63 & -0.21 & -0.93 & 0.73 & 0.60 & 0.22 \\ 
  Mongolian & Mongolic & Mongolian & 0.29 & 0.36 & 0.48 & -0.25 & -0.85 & 0.80 & 0.62 & 0.29 \\ 
  Kinyarwanda & Niger-Congo & Latin & 0.27 & 0.44 & 0.72 & -0.21 & -0.89 & 0.60 & 0.61 & 0.23 \\ 
  Hakha Chin & Sino-Tibetan & Latin & 0.22 & 0.29 & 0.44 & -0.25 & -0.83 & 0.76 & 0.69 & 0.30 \\ 
  Chuvash & Turkic & Cyrillic & 0.38 & 0.45 & 0.55 & -0.25 & -0.82 & 0.83 & 0.56 & 0.30 \\ 
  Kirghiz & Turkic & Cyrillic & 0.34 & 0.44 & 0.57 & -0.19 & -0.89 & 0.78 & 0.56 & 0.22 \\ 
  Tatar & Turkic & Cyrillic & 0.30 & 0.38 & 0.52 & -0.25 & -0.88 & 0.79 & 0.63 & 0.29 \\ 
  Yakut & Turkic & Cyrillic & 0.35 & 0.43 & 0.54 & -0.25 & -0.72 & 0.80 & 0.55 & 0.35 \\ 
  Turkish & Turkic & Latin & 0.32 & 0.41 & 0.55 & -0.21 & -0.89 & 0.78 & 0.59 & 0.23 \\ 
  Estonian & Uralic & Latin & 0.32 & 0.40 & 0.58 & -0.22 & -0.82 & 0.80 & 0.70 & 0.27 \\ 
   \hline


==> tables/omega_tau_omega_ro_cv.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Wed Jun 22 15:10:18 2022
Esperanto &  & Latin & -0.17 & -0.22 & -0.92 & -0.97 & 0.19 & 0.23 \\ 
  Interlingua &  & Latin & -0.23 & -0.29 & -0.79 & -0.88 & 0.29 & 0.33 \\ 
  Arabic & Afro-Asiatic & Arabic & -0.15 & -0.18 & -0.86 & -0.93 & 0.17 & 0.20 \\ 
  Maltese & Afro-Asiatic & Latin & -0.19 & -0.24 & -0.81 & -0.90 & 0.24 & 0.27 \\ 
  Vietnamese & Austroasiatic & Latin & -0.16 & -0.18 & -0.72 & -0.78 & 0.22 & 0.23 \\ 
  Indonesian & Austronesian & Latin & -0.20 & -0.26 & -0.91 & -0.97 & 0.22 & 0.27 \\ 
  Tamil & Dravidian & Tamil & -0.26 & -0.33 & -0.87 & -0.94 & 0.30 & 0.35 \\ 
  Panjabi & Indo-European & Arabic & -0.34 & -0.39 & -0.48 & -0.53 & 0.71 & 0.73 \\ 
  Persian & Indo-European & Arabic & -0.20 & -0.27 & -0.92 & -0.98 & 0.22 & 0.28 \\ 
  Assamese & Indo-European & Assamese & -0.30 & -0.36 & -0.66 & -0.75 & 0.46 & 0.48 \\ 
  Russian & Indo-European & Cyrillic & -0.13 & -0.18 & -0.94 & -0.98 & 0.14 & 0.18 \\ 
  Ukrainian & Indo-European & Cyrillic & -0.16 & -0.21 & -0.86 & -0.93 & 0.19 & 0.22 \\ 
  Modern Greek & Indo-European & Greek & -0.24 & -0.30 & -0.85 & -0.92 & 0.29 & 0.33 \\ 
  Breton & Indo-European & Latin & -0.24 & -0.30 & -0.90 & -0.96 & 0.26 & 0.31 \\ 
  Catalan & Indo-European & Latin & -0.15 & -0.21 & -0.92 & -0.98 & 0.17 & 0.21 \\ 
  Czech & Indo-European & Latin & -0.22 & -0.29 & -0.92 & -0.97 & 0.24 & 0.29 \\ 
  Dutch & Indo-European & Latin & -0.27 & -0.37 & -0.95 & -0.99 & 0.29 & 0.37 \\ 
  English & Indo-European & Latin & -0.07 & -0.09 & -0.83 & -0.91 & 0.09 & 0.10 \\ 
  French & Indo-European & Latin & -0.04 & -0.05 & -0.84 & -0.92 & 0.04 & 0.05 \\ 
  German & Indo-European & Latin & -0.11 & -0.15 & -0.87 & -0.94 & 0.13 & 0.16 \\ 
  Irish & Indo-European & Latin & -0.21 & -0.28 & -0.93 & -0.98 & 0.23 & 0.28 \\ 
  Italian & Indo-European & Latin & -0.05 & -0.07 & -0.90 & -0.96 & 0.06 & 0.07 \\ 
  Latvian & Indo-European & Latin & -0.25 & -0.31 & -0.73 & -0.82 & 0.35 & 0.38 \\ 
  Polish & Indo-European & Latin & -0.17 & -0.23 & -0.94 & -0.98 & 0.18 & 0.23 \\ 
  Portuguese & Indo-European & Latin & -0.18 & -0.24 & -0.91 & -0.96 & 0.20 & 0.25 \\ 
  Romanian & Indo-European & Latin & -0.21 & -0.26 & -0.78 & -0.86 & 0.27 & 0.30 \\ 
  Romansh & Indo-European & Latin & -0.23 & -0.29 & -0.79 & -0.88 & 0.29 & 0.33 \\ 
  Slovenian & Indo-European & Latin & -0.21 & -0.26 & -0.87 & -0.94 & 0.24 & 0.27 \\ 
  Spanish & Indo-European & Latin & -0.03 & -0.04 & -0.91 & -0.97 & 0.03 & 0.04 \\ 
  Swedish & Indo-European & Latin & -0.28 & -0.36 & -0.90 & -0.96 & 0.31 & 0.37 \\ 
  Welsh & Indo-European & Latin & -0.20 & -0.26 & -0.91 & -0.97 & 0.22 & 0.27 \\ 
  Western Frisian & Indo-European & Latin & -0.28 & -0.36 & -0.80 & -0.88 & 0.36 & 0.40 \\ 
  Oriya & Indo-European & Odia & -0.32 & -0.38 & -0.70 & -0.79 & 0.46 & 0.48 \\ 
  Dhivehi & Indo-European & Thaana & -0.23 & -0.29 & -0.82 & -0.88 & 0.28 & 0.33 \\ 
  Georgian & Kartvelian & Georgian & -0.11 & -0.14 & -0.67 & -0.76 & 0.17 & 0.18 \\ 
  Basque & Language isolate & Latin & -0.16 & -0.22 & -0.91 & -0.97 & 0.18 & 0.22 \\ 
  Mongolian & Mongolic & Mongolian & -0.22 & -0.28 & -0.86 & -0.93 & 0.26 & 0.30 \\ 
  Kinyarwanda & Niger-Congo & Latin & -0.19 & -0.25 & -0.90 & -0.96 & 0.21 & 0.26 \\ 
  Abkhazian & Northwest Caucasian & Cyrillic & -0.33 & -0.39 & -0.52 & -0.60 & 0.64 & 0.65 \\ 
  Hakha Chin & Sino-Tibetan & Latin & -0.29 & -0.35 & -0.81 & -0.90 & 0.35 & 0.39 \\ 
  Chuvash & Turkic & Cyrillic & -0.20 & -0.25 & -0.83 & -0.91 & 0.25 & 0.28 \\ 
  Kirghiz & Turkic & Cyrillic & -0.19 & -0.25 & -0.89 & -0.95 & 0.22 & 0.26 \\ 
  Tatar & Turkic & Cyrillic & -0.24 & -0.30 & -0.88 & -0.95 & 0.27 & 0.32 \\ 
  Yakut & Turkic & Cyrillic & -0.26 & -0.32 & -0.74 & -0.83 & 0.35 & 0.39 \\ 
  Turkish & Turkic & Latin & -0.22 & -0.28 & -0.89 & -0.95 & 0.24 & 0.29 \\ 
  Estonian & Uralic & Latin & -0.23 & -0.29 & -0.83 & -0.92 & 0.28 & 0.31 \\ 
   \hline


==> tables/omega_tau_omega_ro_pud.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Tue Aug 30 17:38:54 2022
 Arabic & Afro-Asiatic & Arabic & -0.13 & -0.15 & -0.72 & -0.81 & 0.18 & 0.19 \\ 
  Indonesian & Austronesian & Latin & -0.11 & -0.14 & -0.80 & -0.88 & 0.14 & 0.15 \\ 
  Russian & Indo-European & Cyrillic & -0.19 & -0.23 & -0.64 & -0.73 & 0.30 & 0.32 \\ 
  Hindi & Indo-European & Devanagari & -0.19 & -0.23 & -0.78 & -0.86 & 0.24 & 0.27 \\ 
  Czech & Indo-European & Latin & -0.22 & -0.27 & -0.67 & -0.75 & 0.34 & 0.36 \\ 
  English & Indo-European & Latin & -0.20 & -0.24 & -0.76 & -0.85 & 0.26 & 0.29 \\ 
  French & Indo-European & Latin & -0.17 & -0.21 & -0.76 & -0.84 & 0.22 & 0.24 \\ 
  German & Indo-European & Latin & -0.23 & -0.28 & -0.68 & -0.78 & 0.34 & 0.36 \\ 
  Icelandic & Indo-European & Latin & -0.26 & -0.32 & -0.66 & -0.75 & 0.40 & 0.42 \\ 
  Italian & Indo-European & Latin & -0.18 & -0.22 & -0.76 & -0.84 & 0.23 & 0.26 \\ 
  Polish & Indo-European & Latin & -0.19 & -0.23 & -0.64 & -0.73 & 0.29 & 0.31 \\ 
  Portuguese & Indo-European & Latin & -0.18 & -0.22 & -0.74 & -0.83 & 0.25 & 0.27 \\ 
  Spanish & Indo-European & Latin & -0.16 & -0.20 & -0.74 & -0.83 & 0.22 & 0.24 \\ 
  Swedish & Indo-European & Latin & -0.23 & -0.28 & -0.68 & -0.77 & 0.34 & 0.36 \\ 
  Japanese & Japonic & Japanese & -0.21 & -0.25 & -0.60 & -0.67 & 0.35 & 0.37 \\ 
  Japanese-strokes & Japonic & Japanese & -0.09 & -0.12 & -0.78 & -0.87 & 0.12 & 0.13 \\ 
  Japanese-romaji & Japonic & Latin & -0.15 & -0.19 & -0.80 & -0.87 & 0.19 & 0.21 \\ 
  Korean & Koreanic & Hangul & -0.24 & -0.27 & -0.64 & -0.71 & 0.38 & 0.39 \\ 
  Thai & Kra-Dai & Thai & -0.23 & -0.29 & -0.82 & -0.90 & 0.28 & 0.32 \\ 
  Chinese & Sino-Tibetan & Han (Traditional variant) & -0.24 & -0.27 & -0.55 & -0.59 & 0.44 & 0.45 \\ 
  Chinese-strokes & Sino-Tibetan & Han (Traditional variant) & -0.18 & -0.24 & -0.77 & -0.87 & 0.24 & 0.27 \\ 
  Chinese-pinyin & Sino-Tibetan & Latin & -0.18 & -0.21 & -0.77 & -0.85 & 0.23 & 0.25 \\ 
  Turkish & Turkic & Latin & -0.24 & -0.29 & -0.66 & -0.76 & 0.36 & 0.38 \\ 
  Finnish & Uralic & Latin & -0.23 & -0.28 & -0.60 & -0.69 & 0.39 & 0.41 \\ 
   \hline


==> tables/omega_tau_omega_rocv.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Wed Jun 22 15:01:13 2022
  \hline
Abkhazian & Northwest Caucasian & Cyrillic & -0.33 & -0.39 & -0.52 & -0.60 & 0.64 & 0.65 \\ 
  Arabic & Afro-Asiatic & Arabic & -0.15 & -0.18 & -0.86 & -0.93 & 0.17 & 0.20 \\ 
  Assamese & Indo-European & Assamese & -0.30 & -0.36 & -0.66 & -0.75 & 0.46 & 0.48 \\ 
  Basque & Language isolate & Latin & -0.16 & -0.22 & -0.91 & -0.97 & 0.18 & 0.22 \\ 
  Breton & Indo-European & Latin & -0.24 & -0.30 & -0.90 & -0.96 & 0.26 & 0.31 \\ 
  Catalan & Indo-European & Latin & -0.15 & -0.21 & -0.92 & -0.98 & 0.17 & 0.21 \\ 
  Chuvash & Turkic & Cyrillic & -0.20 & -0.25 & -0.83 & -0.91 & 0.25 & 0.28 \\ 
  Czech & Indo-European & Latin & -0.22 & -0.29 & -0.92 & -0.97 & 0.24 & 0.29 \\ 
  Dhivehi & Indo-European & Thaana & -0.23 & -0.29 & -0.82 & -0.88 & 0.28 & 0.33 \\ 
  Dutch & Indo-European & Latin & -0.27 & -0.37 & -0.95 & -0.99 & 0.29 & 0.37 \\ 
  English & Indo-European & Latin & -0.07 & -0.09 & -0.83 & -0.91 & 0.09 & 0.10 \\ 
  Esperanto &  & Latin & -0.17 & -0.22 & -0.92 & -0.97 & 0.19 & 0.23 \\ 
  Estonian & Uralic & Latin & -0.23 & -0.29 & -0.83 & -0.92 & 0.28 & 0.31 \\ 
  French & Indo-European & Latin & -0.04 & -0.05 & -0.84 & -0.92 & 0.04 & 0.05 \\ 
  Georgian & Kartvelian & Georgian & -0.11 & -0.14 & -0.67 & -0.76 & 0.17 & 0.18 \\ 
  German & Indo-European & Latin & -0.11 & -0.15 & -0.87 & -0.94 & 0.13 & 0.16 \\ 
  Hakha Chin & Sino-Tibetan & Latin & -0.29 & -0.35 & -0.81 & -0.90 & 0.35 & 0.39 \\ 
  Indonesian & Austronesian & Latin & -0.20 & -0.26 & -0.91 & -0.97 & 0.22 & 0.27 \\ 
  Interlingua &  & Latin & -0.23 & -0.29 & -0.79 & -0.88 & 0.29 & 0.33 \\ 
  Irish & Indo-European & Latin & -0.21 & -0.28 & -0.93 & -0.98 & 0.23 & 0.28 \\ 
  Italian & Indo-European & Latin & -0.05 & -0.07 & -0.90 & -0.96 & 0.06 & 0.07 \\ 
  Kinyarwanda & Niger-Congo & Latin & -0.19 & -0.25 & -0.90 & -0.96 & 0.21 & 0.26 \\ 
  Kirghiz & Turkic & Cyrillic & -0.19 & -0.25 & -0.89 & -0.95 & 0.22 & 0.26 \\ 
  Latvian & Indo-European & Latin & -0.25 & -0.31 & -0.73 & -0.82 & 0.35 & 0.38 \\ 
  Maltese & Afro-Asiatic & Latin & -0.19 & -0.24 & -0.81 & -0.90 & 0.24 & 0.27 \\ 
  Modern Greek & Indo-European & Greek & -0.24 & -0.30 & -0.85 & -0.92 & 0.29 & 0.33 \\ 
  Mongolian & Mongolic & Mongolian & -0.22 & -0.28 & -0.86 & -0.93 & 0.26 & 0.30 \\ 
  Oriya & Indo-European & Odia & -0.32 & -0.38 & -0.70 & -0.79 & 0.46 & 0.48 \\ 
  Panjabi & Indo-European & Arabic & -0.34 & -0.39 & -0.48 & -0.53 & 0.71 & 0.73 \\ 
  Persian & Indo-European & Arabic & -0.20 & -0.27 & -0.92 & -0.98 & 0.22 & 0.28 \\ 
  Polish & Indo-European & Latin & -0.17 & -0.23 & -0.94 & -0.98 & 0.18 & 0.23 \\ 
  Portuguese & Indo-European & Latin & -0.18 & -0.24 & -0.91 & -0.96 & 0.20 & 0.25 \\ 
  Romanian & Indo-European & Latin & -0.21 & -0.26 & -0.78 & -0.86 & 0.27 & 0.30 \\ 
  Romansh & Indo-European & Latin & -0.23 & -0.29 & -0.79 & -0.88 & 0.29 & 0.33 \\ 
  Russian & Indo-European & Cyrillic & -0.13 & -0.18 & -0.94 & -0.98 & 0.14 & 0.18 \\ 
  Slovenian & Indo-European & Latin & -0.21 & -0.26 & -0.87 & -0.94 & 0.24 & 0.27 \\ 
  Spanish & Indo-European & Latin & -0.03 & -0.04 & -0.91 & -0.97 & 0.03 & 0.04 \\ 
  Swedish & Indo-European & Latin & -0.28 & -0.36 & -0.90 & -0.96 & 0.31 & 0.37 \\ 
  Tamil & Dravidian & Tamil & -0.26 & -0.33 & -0.87 & -0.94 & 0.30 & 0.35 \\ 
  Tatar & Turkic & Cyrillic & -0.24 & -0.30 & -0.88 & -0.95 & 0.27 & 0.32 \\ 
  Turkish & Turkic & Latin & -0.22 & -0.28 & -0.89 & -0.95 & 0.24 & 0.29 \\ 
  Ukrainian & Indo-European & Cyrillic & -0.16 & -0.21 & -0.86 & -0.93 & 0.19 & 0.22 \\ 
  Vietnamese & Austroasiatic & Latin & -0.16 & -0.18 & -0.72 & -0.78 & 0.22 & 0.23 \\ 
  Welsh & Indo-European & Latin & -0.20 & -0.26 & -0.91 & -0.97 & 0.22 & 0.27 \\ 
  Western Frisian & Indo-European & Latin & -0.28 & -0.36 & -0.80 & -0.88 & 0.36 & 0.40 \\ 
  Yakut & Turkic & Cyrillic & -0.26 & -0.32 & -0.74 & -0.83 & 0.35 & 0.39 \\ 
   \hline


==> tables/omega_tau_omega_ropud.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Wed Jun 22 15:01:13 2022
  \hline
Arabic & Indo-European & Arabic & -0.13 & -0.15 & -0.73 & -0.81 & 0.18 & 0.19 \\ 
  Chinese & Sino-Tibetan & Chinese & -0.24 & -0.27 & -0.76 & -0.87 & 0.32 & 0.31 \\ 
  Chinese-strokes & Sino-Tibetan & Chinese & -0.05 & -0.06 & -0.76 & -0.87 & 0.07 & 0.07 \\ 
  Czech & Indo-European & Latin & -0.22 & -0.26 & -0.66 & -0.74 & 0.33 & 0.35 \\ 
  English & Indo-European & Latin & -0.19 & -0.24 & -0.76 & -0.84 & 0.26 & 0.28 \\ 
  Finnish & Uralic & Latin & -0.23 & -0.27 & -0.59 & -0.68 & 0.39 & 0.40 \\ 
  French & Indo-European & Latin & -0.16 & -0.20 & -0.75 & -0.83 & 0.21 & 0.24 \\ 
  German & Indo-European & Latin & -0.23 & -0.28 & -0.68 & -0.77 & 0.33 & 0.36 \\ 
  Hindi & Indo-European & Devanagari & -0.18 & -0.22 & -0.77 & -0.86 & 0.23 & 0.26 \\ 
  Icelandic & Indo-European & Latin & -0.26 & -0.31 & -0.66 & -0.75 & 0.39 & 0.41 \\ 
  Indonesian & Indo-European & Latin & -0.10 & -0.13 & -0.79 & -0.88 & 0.13 & 0.15 \\ 
  Italian & Indo-European & Latin & -0.16 & -0.20 & -0.74 & -0.83 & 0.22 & 0.24 \\ 
  Japanese & Japonic & Kanji-Kana & -0.21 & -0.24 & -0.78 & -0.87 & 0.27 & 0.28 \\ 
  Japanese-strokes & Japonic & Kanji-Kana & -0.09 & -0.12 & -0.78 & -0.87 & 0.12 & 0.13 \\ 
  Korean & Koreanic & Hangul & -0.24 & -0.27 & -0.64 & -0.71 & 0.37 & 0.38 \\ 
  Polish & Indo-European & Latin & -0.18 & -0.22 & -0.64 & -0.73 & 0.29 & 0.30 \\ 
  Portuguese & Indo-European & Latin & -0.18 & -0.22 & -0.74 & -0.83 & 0.25 & 0.27 \\ 
  Russian & Indo-European & Cyrillic & -0.19 & -0.23 & -0.64 & -0.73 & 0.30 & 0.32 \\ 
  Spanish & Indo-European & Latin & -0.16 & -0.20 & -0.74 & -0.83 & 0.22 & 0.24 \\ 
  Swedish & Indo-European & Latin & -0.23 & -0.27 & -0.68 & -0.77 & 0.33 & 0.35 \\ 
  Thai & Tai-Kadai & Thai & -0.23 & -0.29 & -0.82 & -0.90 & 0.28 & 0.32 \\ 
  Turkish & Turkic & Latin & -0.23 & -0.28 & -0.66 & -0.76 & 0.35 & 0.37 \\ 
   \hline


==> tables/opt_scores_summary_eta.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Jul 28 12:21:13 2022
  & PUD-characters & 0.69 & 0.78 & 0.81 & 0.81 & 0.85 & 0.88 & 0.05 \\ 
   & CV-characters & 0.52 & 0.69 & 0.75 & 0.73 & 0.80 & 0.96 & 0.10 \\ 
   & CV-duration & 0.46 & 0.72 & 0.76 & 0.76 & 0.81 & 0.92 & 0.09 \\ 
   \hline


==> tables/opt_scores_summary_eta_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:22 2022
 & PUD-characters & 0.69 & 0.77 & 0.79 & 0.80 & 0.85 & 0.88 & 0.05 \\ 
   & CV-characters & 0.51 & 0.68 & 0.75 & 0.73 & 0.80 & 0.97 & 0.11 \\ 
   & CV-duration & 0.50 & 0.71 & 0.76 & 0.76 & 0.81 & 0.93 & 0.09 \\ 
   \hline


==> tables/opt_scores_summary_null_eta.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Sep  8 15:04:05 2022
  & PUD-characters & 0.477 & 0.521 & 0.551 & 0.580 & 0.646 & 0.747 & 0.081 \\ 
   & CV-characters & 0.268 & 0.423 & 0.495 & 0.518 & 0.575 & 0.915 & 0.145 \\ 
   & CV-duration & 0.213 & 0.426 & 0.504 & 0.518 & 0.603 & 0.882 & 0.139 \\ 
   \hline


==> tables/opt_scores_summary_null_eta_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:12 2022
 & PUD-characters & 0.453 & 0.504 & 0.553 & 0.575 & 0.647 & 0.747 & 0.082 \\ 
   & CV-characters & 0.284 & 0.423 & 0.493 & 0.518 & 0.576 & 0.915 & 0.147 \\ 
   & CV-duration & 0.234 & 0.424 & 0.505 & 0.518 & 0.604 & 0.888 & 0.144 \\ 
   \hline


==> tables/opt_scores_summary_null_omega.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Sep  8 15:04:05 2022
  & PUD-characters & -0.000 & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-characters & -0.000 & -0.000 & 0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-duration & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \hline


==> tables/opt_scores_summary_null_omega_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:12 2022
 & PUD-characters & -0.000 & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-characters & -0.000 & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-duration & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \hline


==> tables/opt_scores_summary_null_psi.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Sep  8 15:04:05 2022
  & PUD-characters & -0.000 & -0.000 & 0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-characters & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-duration & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.001 & 0.000 \\ 
   \hline


==> tables/opt_scores_summary_null_psi_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:12 2022
 & PUD-characters & -0.000 & -0.000 & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-characters & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   & CV-duration & -0.000 & -0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \hline


==> tables/opt_scores_summary_omega.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Jul 28 12:21:13 2022
  & PUD-characters & 0.13 & 0.23 & 0.29 & 0.29 & 0.35 & 0.44 & 0.08 \\ 
   & CV-characters & 0.04 & 0.19 & 0.24 & 0.26 & 0.30 & 0.68 & 0.12 \\ 
   & CV-duration & 0.09 & 0.22 & 0.25 & 0.26 & 0.31 & 0.45 & 0.07 \\ 
   \hline


==> tables/opt_scores_summary_omega_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:22 2022
 & PUD-characters & 0.13 & 0.22 & 0.28 & 0.29 & 0.35 & 0.44 & 0.08 \\ 
   & CV-characters & 0.03 & 0.19 & 0.24 & 0.25 & 0.29 & 0.71 & 0.13 \\ 
   & CV-duration & 0.08 & 0.22 & 0.25 & 0.26 & 0.30 & 0.46 & 0.08 \\ 
   \hline


==> tables/opt_scores_summary_psi.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Jul 28 12:21:13 2022
  & PUD-characters & 0.42 & 0.64 & 0.70 & 0.67 & 0.72 & 0.78 & 0.08 \\ 
   & CV-characters & 0.33 & 0.57 & 0.63 & 0.62 & 0.68 & 0.79 & 0.09 \\ 
   & CV-duration & 0.33 & 0.60 & 0.69 & 0.66 & 0.73 & 0.83 & 0.11 \\ 
   \hline


==> tables/opt_scores_summary_psi_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Tue Jul  5 15:43:22 2022
 & PUD-characters & 0.42 & 0.64 & 0.69 & 0.67 & 0.71 & 0.78 & 0.08 \\ 
   & CV-characters & 0.26 & 0.56 & 0.63 & 0.62 & 0.68 & 0.79 & 0.09 \\ 
   & CV-duration & 0.30 & 0.60 & 0.69 & 0.65 & 0.72 & 0.83 & 0.11 \\ 
   \hline


==> tables/pud_opt_scores_characters_kendall.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
% Mon Jul 11 12:37:22 2022
 Arabic & Afro-Asiatic & Arabic & 3.39 & 4.16 & 5.56 & -0.13 & -0.72 & 0.82 & 0.65 & 0.18 \\ 
  Indonesian & Austronesian & Latin & 4.13 & 5.98 & 7.34 & -0.10 & -0.79 & 0.69 & 0.42 & 0.13 \\ 
  Russian & Indo-European & Cyrillic & 5.19 & 6.04 & 8.08 & -0.19 & -0.64 & 0.86 & 0.70 & 0.30 \\ 
  Hindi & Indo-European & Devanagari & 3.12 & 4.11 & 5.83 & -0.18 & -0.77 & 0.76 & 0.64 & 0.23 \\ 
  Czech & Indo-European & Latin & 4.72 & 5.46 & 7.25 & -0.22 & -0.66 & 0.86 & 0.71 & 0.33 \\ 
  English & Indo-European & Latin & 3.79 & 4.87 & 6.99 & -0.19 & -0.76 & 0.78 & 0.66 & 0.26 \\ 
  French & Indo-European & Latin & 3.69 & 4.81 & 7.47 & -0.16 & -0.75 & 0.77 & 0.70 & 0.21 \\ 
  German & Indo-European & Latin & 4.53 & 5.75 & 8.55 & -0.23 & -0.68 & 0.79 & 0.70 & 0.33 \\ 
  Icelandic & Indo-European & Latin & 4.44 & 5.33 & 7.88 & -0.26 & -0.66 & 0.83 & 0.74 & 0.39 \\ 
  Italian & Indo-European & Latin & 3.80 & 4.85 & 7.63 & -0.16 & -0.74 & 0.78 & 0.73 & 0.22 \\ 
  Polish & Indo-European & Latin & 5.16 & 6.07 & 7.97 & -0.18 & -0.64 & 0.85 & 0.68 & 0.29 \\ 
  Portuguese & Indo-European & Latin & 3.57 & 4.53 & 7.48 & -0.18 & -0.74 & 0.79 & 0.75 & 0.25 \\ 
  Spanish & Indo-European & Latin & 3.74 & 4.83 & 7.59 & -0.16 & -0.74 & 0.77 & 0.72 & 0.22 \\ 
  Swedish & Indo-European & Latin & 4.31 & 5.43 & 7.96 & -0.23 & -0.68 & 0.79 & 0.69 & 0.33 \\ 
  Japanese & Japonic & Japanese & 1.45 & 1.73 & 2.71 & -0.21 & -0.60 & 0.84 & 0.78 & 0.35 \\ 
  Japanese-strokes & Japonic & Japanese & 5.17 & 7.73 & 13.94 & -0.09 & -0.78 & 0.67 & 0.71 & 0.12 \\ 
  Japanese-romaji & Japonic & Latin & 2.75 & 3.84 & 6.09 & -0.16 & -0.80 & 0.72 & 0.67 & 0.20 \\ 
  Korean & Koreanic & Hangul & 2.38 & 2.72 & 3.19 & -0.24 & -0.64 & 0.88 & 0.59 & 0.37 \\ 
  Thai & Kra-Dai & Thai & 3.19 & 4.37 & 6.37 & -0.23 & -0.82 & 0.73 & 0.63 & 0.28 \\ 
  Chinese & Sino-Tibetan & Han (Simplified variant) & 1.47 & 1.67 & 2.18 & -0.24 & -0.55 & 0.88 & 0.72 & 0.44 \\ 
  Chinese-strokes & Sino-Tibetan & Han (Simplified variant) & 3.25 & 6.83 & 7.89 & -0.05 & -0.76 & 0.48 & 0.23 & 0.07 \\ 
  Chinese-pinyin & Sino-Tibetan & Latin & 3.88 & 4.93 & 6.58 & -0.17 & -0.77 & 0.79 & 0.61 & 0.22 \\ 
  Turkish & Turkic & Latin & 5.35 & 6.43 & 7.92 & -0.23 & -0.66 & 0.83 & 0.58 & 0.35 \\ 
  Finnish & Uralic & Latin & 6.55 & 7.51 & 9.27 & -0.23 & -0.59 & 0.87 & 0.65 & 0.39 \\ 
   \hline

